Measuring the Impact of Influence on Individuals: Roadmap to Quantifying Attitude

Influence diffusion has been central to the study of propagation of information in social networks, where influence is typically modeled as a binary property of entities: influenced or not influenced. We introduce the notion of attitude, which, as described in social psychology, is the degree by which an entity is influenced by the information. We present an information diffusion model that quantifies the degree of influence, i.e., attitude of individuals, in a social network. With this model, we formulate and study attitude maximization problem. We prove that the function for computing attitude is monotonic and sub-modular, and the attitude maximization problem is NP-Hard. We present a greedy algorithm for maximization with an approximation guarantee of $(1-1/e)$. Using the same model, we also introduce the notion of "actionable" attitude with the aim to study the scenarios where attaining individuals with high attitude is objectively more important than maximizing the attitude of the entire network. We show that the function for computing actionable attitude, unlike that for computing attitude, is non-submodular and however is \emph{approximately submodular}. We present approximation algorithm for maximizing actionable attitude in a network. We experimentally evaluated our algorithms and study empirical properties of the attitude of nodes in network such as spatial and value distribution of high attitude nodes.

==> plots.tex <==



% \newcommand{\budgetVPlot}[4]{
% \resizebox {0.19\linewidth} {!} {
% \begin{tikzpicture}
%     \begin{axis}[xlabel=\textbf{Budget}, title=\textbf{#3}, legend pos=south east]
%         \pgfplotstableread[col sep=comma]{datasets/#1}
%         \datatablebudget
%         \addlegendimage{empty legend}\addlegendentry{#4}
%         \addplot table[y = #2] from \datatablebudget ;
%     \end{axis}
% \end{tikzpicture}}}




% \begin{figure*}[htp]

% \begin{tabular}{ccccc}

% \budgetVPlot{budgetVsAtt.csv}{facebook}{Attitude}{Facebook}
% &
% \budgetVPlot{budgetVsAtt.csv}{nethept}{Attitude}{NetHept}
% &
% \budgetVPlot{budgetVsAtt.csv}{amazon}{Attitude}{Amazon}
% &
% \budgetVPlot{budgetVsAtt.csv}{dblp}{Attitude}{DBLP}
% &
% \budgetVPlot{budgetVsAtt.csv}{youtube}{Attitude}{Youtube}
% \\

% \budgetVPlot{budgetVsTime.csv}{facebook}{Time Taken}{Facebook}
% &
% \budgetVPlot{budgetVsTime.csv}{nethept}{Time Taken}{NetHept}
% &
% \budgetVPlot{budgetVsTime.csv}{amazon}{Time Taken}{Amazon}
% &
% \budgetVPlot{budgetVsTime.csv}{dblp}{Time Taken}{DBLP}
% &
% \budgetVPlot{budgetVsTime.csv}{youtube}{Time Taken}{Youtube}

% \end{tabular}
% \label{fig:BudgetVs}
% \caption{Experimental results of \attup maximization with $p=0.1$. a) The first row shows the expected \attup b) The second row shows the time taken to find the seed set.}
% \end{figure*}





==> response.tex <==
%% \documentclass[11pt]{article}

%% \usepackage{fullpage,color}

%% \begin{document}

\noindent
\textbf{Response to Reviewer Comments and Suggestions}

We thank the reviewers for many suggestions and comments. All the changes that were made in response to the suggestions are on color \color{blue}.


\medskip
\noindent
\textbf{Reviewer 2.}

%\begin{enumerate}[leftmargin=.5in]
%\item[W1, D1. ]  

\smallskip
\noindent
\textbf{[W1, D1]} The motivation lacks real-world applications,
especially for the problem of attribute maximization. No existing
real-world datasets and results are offered to support this new
model. It needs new experiments to validate the effectiveness of
attributes and also actionable attributes based mathematical models.
%\end{enumerate}

\color{blue} 

Following the existing work, we have included additional experiments
using DBLP data (see Section~7). The objective of these experiments is
to present the relationship between attitude values and contributions
in terms of number of publications; in particular, experimental
results indicate that higher attitude indicates higher publications.
Note that, binary properties, such as influenced or not, cannot reveal
such relative ordering in terms of publications.

\color{black}


%\item[W2, D2. ]

\smallskip 
\noindent
\textbf{[W2, D2]}
Techniques seem to have limited contributions and similar
  results as IM, in which the challenges of investigating new problems
  are not clear. Several function properties and techniques seem to be not
  very surprising extending from IM to the new problem, e.g.,
  NP-hardness, submodularity, (1-1/e)-approximation, and RR Set.


\color{blue} 

Conceptually, the primary contribution of this work is to arrive at a mathematical model to capture ``attitude''--strength of the influence. This model takes a cue from social psychology that distinguishes between belief (influence) and  attitude. The work in this field postulates that repeated exposure can increase the attitude. The proposed model is based on the suggestions and postulates from sociology.

Once the model is defined, a {\em critical technical contribution} is Theorem 2. This theorem presents a relationship between expected attitude the expected number of activated edges. A priori, its is difficult to fathom that attitude can be captured using expected number of live edges.   In our view, this is one of those theorems that is  easy/not surprising in hindsight.  Once stated, it is intuitive.  This characterization forms the basis for the computation techniques and theoretical results for attitude maximization problem [Theorems 2,
  3, 4 and 5].
  
We agree with that once we have this characterization, submodularity, monotonicity, and usage of RR set based techniques are not that surprising. While it is reasonable to expect that RR sets can be used to design algorithms, there are few small subtleties  that need to be taken care of. For example, for influence computation, RR set generation starts by randomly picking a node, and this idea does not work here. We need to start by randomly picking an edge $e$, keep that edge with probability $p(e)$, if the edge is kept then only generation of RR set proceeds. Such details cannot be overlooked, and thus we provided complete proofs. 

%Our primary contribution is in the modeling strategy for quantifying
%the number of repeated exposure (which we refer to as
%\emph{attitude}). It is not immediate that the expected attitude is
%directly proportional to the number of activated edges in the
%influence graph. This forms 
%First, the relationship with the number of activated edges is utilized
%in attitude computation using reverse sampling method (with
%modification that the sampling starts with a random selection of edge
%rather than a node) [Theorems 6, 7; and Lemma 2]. 

Second, the hardness of attitude maximization problem follows by giving a reduction to the influence maximization problem, and the reduction while not overly difficult is not obvious either. As with many NP-completeness proofs, we need the correct ``gadget'' to arrive at the reduction. There is a key extension
to the construction which strategically incorporates the relationship
between activated edges and attitude [Theorem 8]. 

Finally, the theoretical results corresponding to actionable attitude
do not follow from any prior results on influence maximization. While
the (1-1/e)-approximation holds for attitude maximization problem, the(
function for actionable attitude computation does not satisfy the
submodular property (that renders approximation guarantees for
influence maximization and attitude maximization).

We believe that realizing that  the actionable attitude function is ``close to being submodular'' and capturing the closeness with {\em almost submodularity } is an interesting conceptual as well as technical contribution.  To the best of our knowledge, this definition of almost submodularity is new (though a few other versions of approximate submodularity have been studied).  We showed that the actionable attitude 
function is almost submodular and hence the approximation includes an
additive error dependent on the structure of the network [Theorems 13,
  14]. Moreover, as explained in Section 6 (paragraph after statement of Theorem 14), adapting RR sets approach to actionable attitude is non-trivial. One need to carefully tread between random choice of nodes vs random choice of edges.

Our modeling strategy and objectives are distinct from 
influence maximization and we believe that the results, though
indicate the same hardness and approximation results, do not
immediately follow from the existing influence maximization results.

\color{black}


%\item[W3, D3. ] 

\smallskip
\noindent
\textbf{[W3, D3]}
Experiments are not comprehensive, especially for the
  quality evaluation of the proposed AIC model is missing. Table 3 only shows the three datasets' results. It's
  unclear the comparison results of average attributes on other
  datasets.
%\end{enumerate}

\color{blue}

We included new experiments to evaluate the proposed AIC model. The experiments and the results are discussed in Section 7. We added more data sets to Table 3.

\color{black}
\smallskip
\noindent
\textbf{D4, D6.}  In theorem 9, when $S_a= \{a\}$, the attitude may be 7.  ``Kempe et al --> Kempe et al.''
\color{blue}
Fixed the typos.
color{black}
\smallskip
\noindent
\textbf{D5.} In Section 5, when providing an approximate solution, it needs to give more details on explaining why S can be replaced by S* after applying the Chernoff bounds.
\color{blue}
Fixed a typo in the equality and added explanation.


%\end{enumerate}


\medskip
\noindent
\textbf{Reviewer 3.}

%\begin{enumerate}

%\item[W1.] 

\smallskip
\noindent
\textbf{[W1]} The overall framework (algorithm design, hardness
proofs, quality guarantees) is quite similar to the RSS-based
influence maximization problem that has been extensively
studied. Thus, I find the contribution to be incremental in nature.

\color{blue} 

The objective of our work is different from influence maximization and
hence the model strategy for quantifying attitude as opposed to
influence is different as well.  Though the techniques applied are
similar, the correct application of these techniques (e.g. RSS) and
their guarantees require careful understanding of the properties that
relates to attitude. The contributions of our work is not in the
development of new techniques for influence maximization, rather in
understanding and computing new properties of nodes in a influence
network, that can reveal interesting characteristic of the behavior of
the nodes and the network as a whole.

 Please refer to the W2:D2 for Reviewer 2 above for further details.
\color{black}

%\item[W2, D1.]
\smallskip 
\noindent
\textbf{[W2, D1]}  The concept of "attitude maximization" is not
entirely new, similar problem has been studied in the past, but with
different names.  The concept of "attitude maximization" is not
entirely new, similar problem has been studied in the past, but with
different names.

%\begin{enumerate}
%\item[(A)] Maximizing the Cumulative Influence through a Social
 % Network when Repeat Activation Exists [ICCS 2014]
%% On flow authority discovery in social networks [SDM 2011]
%%  Authority Model in Social Networks [ICDCIT 2014]
%\item[(D)] Improving Efficiency of Maximizing Spread in the Flow
 % Authority Model for Large Sparse Networks [BigData 2014]
%\item[(E)] An Influence Propagation View of PageRank [TKDD 2017]
%\item[(F)] Linear Computation for Independent Social Influence [ICDM
%  2013] 
%\end{enumerate}
%\end{enumerate}
\color{blue} 

We thank the reviewer for providing the references.  We have detailed
discussion of the existing work and present the distinguishing aspect
of our work in Section 2.  We present here an outline of the
discussion.  The primary difference between the existing work and ours
stems from the fact that properties of the nodes are binary
(influence/activated and not-influenced/inactive) and hence the
objectives of the existing work do not align with the objective of our
work.


The work related to \emph{repeat activation} focus on identifying the
number of nodes that can be activated if their (already activated)
neighbors are allowed repeatedly influence them.  While on the
surface, the model appears to be similar to the one presented in our
work, the underlying objective and technical properties are different.
\begin{enumerate}
\item \textit{Binary vs. Numerical Property of nodes.\ } Repeat
  activation will result in two groups of nodes: activated or not
  activated; and, hence, does not distinguish the nodes in terms of
  the number of tries (repeat activation) that lead to activation. On
  the other hand, we focus on number of times an already activated
  node could have received activation signal from the neighbors; we
  refer to this number as \emph{attitude} and differentiate nodes in
  terms of their attitudes.  

\item \emph{Objective.\ } The work on repeat activation identifies the
  nodes that can maximize the number of activated nodes using the
  repeat activation strategy. In this respect, the existing work
  aligns with the influence maximization problems using different
  model for influence propagation.. Our work, on the other hand,
  focuses on maximizing the attitude of the overall network. We have
  illustrated using Figure 1, the influence maximization is different
  from the attitude maximization problem.

\item \emph{Influence propagation.\ } Due to the nature of repeat
  activation, the number of steps in steps of repeat activation is
  bounded; otherwise, activation function can diverge. This is the not
  the case in our propagation model, as only the newly activated nodes
  may be able to improve the attitude of its neighbor.
\end{enumerate}

\smallskip

The other line of work referred by the reviewer is based on PageRank
algorithms, where the influence of one node on another depends on the
linear combination of influence of the former on the neighbors of the
latter. This is a generalization of standard influence propagation
models (such as IC model). The objective of this modeling strategy is
to identify the nodes that are influenced; which, as noted above, is
different from the objective of our work: identify the number of times
an influenced node is exposed to the (influential) information.

\smallskip
In flow authority model, any activated node is allowed to activate its
inactive neighbors till a steady state is reached. The model is used
to quantify the \emph{liveness} of information in the network; where
at each iterations nodes that are least likely to be exposed to the
information (repeated exposure) are discarded. The objective is to
find the nodes which can maximize the flow of information in the
network. In contrast, our work focuses on improving the attitude of
the network. It can be interesting to analyze the conjecture the nodes
that maximizes the attitude also maximizes the flow of the information
in the network or vice versa; however, our understanding of the flow
authority work do not indicate the theoretical validity of such
relationship.



\color{black}

%\item[D2.]
\smallskip 
\noindent
\textbf{[D2]} 
RSS is not the most efficient (nor state-of-the-art)
  influence maximization model. As the proposed algorithm is based on
  RSS, it will also suffer from the limitations of RSS, such as high
  memory usage. These points are not experimentally demonstrated,
  neither discussed. Moreover, what about the applicability of the
  more recent IM algorithms in solving the current problem?

\color{blue} 

As a first step, we have used RSS to realize a technique that has
provable guarantees. There are several heuristics that have been
developed and compared in the context of influence
maximization. However, such heuristics, typically, do not provide
guarantees and their characterization (in terms of quality) solely
depends on extensive experimental data analysis, which, in turn,
requires considerable understanding of the structure of the data and
the possible implications of such structure on the heuristics. We will
continue with this effort as part of future research plan.

As pointed, RSS suffers with memory usage issues caused by generation of a large number of RR sets.
Prior works showed that such issues can be addressed by enhancing RSS algorithms Stop-and-stare algorithm that attempts to generate ``optimal'' number of RR sets. In our experiments (for the original submitted version), we used this approach. In the current version, we explicitly pointed this at the beginning of Section 7.

In the current paper, we have been able to present experimental results for
networks of different sizes (the largest being the YouTube network
with over 1m nodes and around 3m edges).

We acknowledged the limitation of RR based technique for actionable attitude as the algorithm needs to store and process graphs as opposed to sets (at the end of Section 6 and in experiments on actionable attitude). 


\color{black}

%\end{enumerate}

\medskip
\noindent
\textbf{Reviewer 4.}

%\begin{enumerate}

%\item[R1)]
\smallskip 
\noindent
\textbf{[R1]} 
Explain and justify the meaning of different attitude
  ratings and how they relate to each other. Especially, explain what
  an attitude of 0 exactly means. (See D1)

\color{blue} 

The attitude $0$ means that a node has not been influenced or
activated. Such a node cannot influence/activate its neighbors. In
this context, the attitude $0$ is identical to not-influenced
state used in traditional influence maximization problems.

\color{black}

%\item[R2)]
\smallskip 
\noindent
\textbf{[R2]} 
Provide evidence that users who have been influenced twice
  behave differently than those who have only been influenced once
  (actionable vs non-actionable). (See D2)

\color{blue} In our model, the attitude values of the nodes provide a
way to relatively order the nodes. We have conducted additional
experiments using DBLP data to show that relative order induced by
attitude indeed captures the relative order of authors in terms of
their contributions.  Please see Section 7.


We point that a certain attitude value in isolation may not reveal much information.
Rather than the actual attitude value,  the ordering of attitude values provide more insights.
It is worth noting that the absolute difference in attitude values may
not be meaningful.  For instance, if attitude of three authors in DBLP
network are $a_1$ $a_2$ and $a_3$ and $a_1-a_2 = a_2-a_3$, then this
does not imply that the the difference between the contributions of
the first and second authors is identical/proportional to the
difference between the contributions between second and third authors.
These points are made explicit at the start of Section 6 and in Section 7 (in the paragraph {\em Interpreting Attitude Values}).


\color{black}

%\item[R3)]
\smallskip 
\noindent
\textbf{[R3]} 
Improve Definition 3 and provide a simple example. (See D3)

\color{blue} We provided an example.


\color{black}

%\item[R4)]
\smallskip 
\noindent
\textbf{[R4]} 
Fix minor spelling errors. (See D4)

\color{blue} We fixed all spelling and grammatical errors that we found.

%\end{enumerate}
\color{black}

\paragraph*{Meta Review Revision items}

\begin{enumerate}
\item Presentation needs to be significantly improved.
\item Real-world application should be studied and tested.
\item Novelty clarification from existing similar problems should be
  provided. 
\item More experimental results on AIC are desired.
\end{enumerate}
\color{blue}  In the current version, we performed more experiments using real world examples to test the model, included the literature pointed by the reviewers and discussed the similarities and differences between those works and our work. We tried to improve the presentation by fixing grammatical and spelling errors and providing more explanations.


Description of additional experiments and other suggested changes caused the paper to go above 12 pages. Thus we removed a few mathematical derivations.
\color{black}
%%\end{document}

